Mapping Surfaces with Earcut

Mapping a shape to some parametric domain is a fundamental tool in graphics and scientific computing. In practice, a map between two shapes is commonly represented by two meshes with same connectivity and different embedding. The standard approach is to input a meshing of one of the two domains plus a function that projects its boundary to the other domain, and then solve for the position of the interior vertices. Inspired by basic principles in mesh generation, in this paper we present the reader a novel point of view on mesh parameterization: we consider connectivity as an additional unknown, and assume that our inputs are just two boundaries that enclose the domains we want to connect. We compute the map by simultaneously growing the same mesh inside both shapes.This change in perspective allows us to recast the parameterization problem as a mesh generation problem, granting access to a wide set of mature tools that are typically not used in this setting. Our practical outcome is a provably robust yet trivial to implement algorithm that maps any planar shape with simple topology to a homotopic domain that is weakly visible from an inner convex kernel. Furthermore, we speculate on a possible extension of the proposed ideas to volumetric maps, listing the major challenges that arise. Differently from prior methods, for which we show that a volumetric extension is not possible, our analysis leaves us reasoneable hopes that the robust generation of volumetric maps via compatible mesh generation could be obtained in the future.

==> Earcut Mapping - A Mesh Generation Perspective on Robust Parameterizations/01_intro.tex <==
\section{Introduction}
\label{sec:intro}

%  1  What is a simplicial map 
%  2  How this is encoded
%  3  Calssical methods for d=2 and open issues with d=3
%  4  Change of perspective and why we are cool


A one-to-one map between two topological spaces $A$ and $B$ is a function $f : A \leftrightarrow B$ that connects points in both domains. 
%For practical reasons, in scientific computing we are often interested in injective (i.e., $f : A \rightarrow B$) and bijective functions (i.e. $f: A \leftrightarrow B$). 
When it comes to actual coding, the realization of this mathematical idea is typically implemented using simplicial meshes to represent topological spaces.
%, and a shared connectivity to express the mapping function.
%typically involves two meshes. %whose embedding encodes the geometry of the topological spaces, and whose connectivity encodes the mapping function $f$. 
Specifically, given two simplicial complexes $M_A,M_B$ that \emph{discretize} $A$ and $B$, the piece-wise linear map $f_M$ connecting them is implicitly defined by their shared connectivity.
%often comes in the form of a mesh connectivity that is shared by both $M_A$ and $M_B$. 
If both meshes do not 
%self-intersect and do not 
contain degenerate elements, boundaries do not self intersect and all triangles have coherent orientation, there exists a bijection $f_M : M_A \leftrightarrow M_B$ \cite{lipman2014bijective}. In fact, any point $p \in M_A$ is identified by a mesh element and a unique set of barycentric coordinates that locate $p$ inside it. Exploiting the shared connectivity, the image $\tilde{p} = f_M(p)$ can be located in $M_B$ by considering the same mesh element and the same barycentric coordinates. Switching $M_A$ with $M_B$ allows to navigate the map in the opposite direction.
%Similarly, the map can be navigated in the opposite direction just by starting from $M_B$ and using applying the same algorithm just switching the topological spaces.
%This type of mapping is extremely efficient to evaluate, and is also very robust, because it is encoded in the topological structure of the meshes, regardless of the position of their vertices. Assuming the meshes do not contain degenerate elements (e.g. zero area faces, zero length edges), the map is always one-to-one, even if they self-intersect or overlap.

%\item[2)] $M_A$ and $M_B$ have different connectivity but overlap to each other. In this case point correspondences can be computed by taking a point $p \in M_A$, and finding one element $t \in M_B$ mesh that contains it. There may be multiple such elements (image picking a point that is coincident with a vertex of $M_B$, any mesh element incident to such vertex contains $p$). Once the element $t$ is found, solving for the barycentric coordinates of $p$ w.r.t. $T$ gives $f(p)$. The evaluation of this map is computationally more involved than the previous one, because it requires to solve a point location problem -- which is linear in the number of elements in $M_B$ and may go down to logaritmic if a spatial data structure is used -- and also requires to solve for the barycentric coordinates of the wanted point once the containing element is found. Moreover, this map is purely geometric, hence more fragile than the previous one. If a mesh overlaps or self-intersects, than the map is not one-to-one.

Algorithms for the parameterization of a given mesh $M_A$ to some target domain $B$ typically input $M_A$ and the value of $f_M$ for each boundary vertex $p \in \partial M_A$, such that they jointly interpolate the boundary of $B$. Then, these methods internally compute $f_M$ for the interior vertices of the mesh, completing the embedding of $M_B$. The most widely used strategy to accomplish this task amounts to define some energy that encodes the distortion of the map, and then minimize it with numerical optimization. To this end, methods mainly differ for the types of energies they use and the numerical schemes used to minimize them. Despite hugely popular, methods based on numerical optimization suffer from two major problems: (i) they do not allow to edit the input topology, and may operate in an empty feasible space 
%possibly resulting in deadlock configurations which do not admit a valid solution 
(Figure~\ref{fig:no_solution}); (ii) they often require the minimization of highly non linear energies, hence the output results depend on the initialization of the solver and its ability to land on a good local minimum.

In this paper we offer the reader a novel view on the mapping problem, unpinning it from the classical formulation based on numerical optimization. Keeping in mind that the ultimate goal is to produce two meshes that discretize the two domains and also share the same connectivity, we observe that an alternative way to formulate this problem consists in assuming as input two boundary representations of the spaces we want to connect, and to generate the wanted map by \emph{simultaneously growing the same mesh} inside both domains. Differently from prior methods, in this case the amount of interior vertices and the whole mesh connectivity are not fixed a priori, but rather become additional unknowns. This opens the space of solutions, allowing to design a mesh that is not tailored for one space only and then forcefully imposed in the other, but is rather a good compromise for both spaces (Figure~\ref{fig:no_solution}, right). 
%Furthermore, this tiny shift in perspective allows us to recast the parameterization problem as a mesh generation problem, granting access to a wide set of mature tools that are typically not used in this setting. 

%In this document we set the basics principles of the idea, and 
We demonstrate our ideas in the context of planar maps, %. Specifically, we show 
showing how the earcut triangulation algorithm can be used to initialize a provably bijective map between two polygons with simple topology. An earlier version of this paper was published at the international conference Smart Tools and Applications for Graphics, obtaining a honorable mention~\cite{Liv20b}. The proposed algorithm was limited to maps to strictly convex polygons. In this short paper we improve the original method, extending the class of admissible domains to any simple polygon that is weakly visible from a convex inner kernel~\cite{avis1981optimal,valentine1953minimal}. This class is much bigger than the class of convex polygons, and is also bigger than the class of star shaped polygons, which is fully included in it. 
%For this revised version 
We also conducted an extensive validation campaign, testing the new algorithm against more than two thousand shapes with varying complexity.

%The reason why we are still interested at studying novel solutions to this problem (and the main motivation for this work), is that known techniques do not extend to 3d. For the Tutte case this was shown multiple times via counter examples~\cite{chilakamarri1995three,de2003tutte}, but even modern approaches such as Progressive Embeddings~\cite{shen2019progressive} raise major theoretical challenges going one dimension up (Section~\ref{sec:related}). As of today, the problem of initializing a valid simplicial map between two topologial spaces of dimension $d \geq 3$ is still open, and all we have is heuristic solutions that are based on numerical optimization of complex functionals, which do not provide guarantees of success~\cite{du2020lifting,su2019practical}. 

A major motivation for this research
%An interesting aspect which highly motivates this research 
stems form the fact that prior methods for robust 2D mapping do not extend to 3D. For the famous Tutte mapping~\cite{tutte1963draw} 
%Solving the planar mapping problem may not seem particularly exciting, because solutions to it 
%Even if the proposed algorithm works in 2d, this research is mainly motivated by the quest for methods to robustly initialize a volumetric map. 
%Solution to the 2d mapping problem were known already in 1963, when Tutte published his famous article on barycentric mapping~\cite{tutte1963draw}, but prior techniques do not extend to 3d. 
%For the Tutte case 
this was shown multiple times via counter examples~\cite{chilakamarri1995three,de2003tutte}. But even modern approaches such as Progressive Embeddings~\cite{shen2019progressive} raise major theoretical challenges going one dimension up (Section~\ref{sec:related}). 
%As of today, the problem of initializing a valid simplicial map between two volumetric meshes is still open, and all we have is heuristic solutions that are based on numerical optimization of complex functionals, which fail to provide guarantees of success~\cite{du2020lifting,su2019practical}. 
In Section~\ref{sec:conclusions} we speculate on a possible extension of our findings to volume meshes, providing a list of (revised) computational geometry questions that form the theoretical foundation for tetrahedral meshing algorithms, but are still unanswered for the case of simultaneous meshing of two shapes at once. We believe that answering these questions will provide powerful tools to attack the volumetric mapping problem via mesh generation.

\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{img/empty_solution_space}
	\caption{Top left: mapping the left polygon into the right one inevitably flips triangle $ijk$. Bottom left: similar deadlock configurations may also occur for interior vertices (yellow), because the intersection of the feasible cones of its neighbors is empty. Right column: inserting additional vertices in the domain (blue) allows to correctly complete both maps. Topological issues are hard to find with a static analysis of the input mesh, and may cause undefined behavior in the solver.}
	\label{fig:no_solution}
\end{figure}


%The main motivation for this work is that, differently from the Tutte embedding and his children, formulating the mapping problem as a mesh generation problem seems to give rise to a family of algorithms that have potential to scale to higher dimensions. Indeed, going one dimension up raises a number of issues that are not present in 2d (Section~\ref{sec:}), but with this work we  -- but the main motivation for this work is that developing this theory further we could eventually be able to find a robust and theoretically sound solution for the mapping problem in 3d.


%Nonetheless, we argue that it is worth studying this novel approaches because, differently from the Tutte embedding and his successors, 


%Considering the plethora of algorithms for mesh parameterization, one may obviously ask whether a work like this is actually needed. The main argument and source of motivation is that despite provably robust methods for mapping disk-like surfaces were known already in 1963, when Tutte published his famous article on barycentric mapping~\cite{tutte1963draw}, the same does not hold for higher dimensions. In particular, it is widely known due to multiple reported failure cases, that the barycentric mapping does not extend to 3d~\cite{chilakamarri1995three,de2003tutte} and -- as of the time of writing -- the problem of initializing a valid simplicial map between two topologial spaces of dimension $d \geq 3$ is still open. 

%There have been numeroud effortsi
%This problem has been widely investigated over the years, but the definition of a provably correct algorithm is still elusive, and even the most recent methods fail to provide guarantees of success~\cite{du2020lifting}.

%Considering that simplicial mesh generation tools are quite mature both in 2d and 3d, we believe that this machinery has good




%This may not sound particularly exciting, because solutions to this problem were known already in 1963, when tutte Tutte published his famous article on barycentric mapping~\cite{tutte1963draw}. However,  





%there are dozens of algorithms that can do it, the nice news is that this approach \emph{seems} to have potential to scale to 3D with minimal edits. This would allow to solve a problem that is still open, namely the provably robust initialization of simplicial maps in 3D. In Section~\ref{sec:results} we dive into the details of this topic, also discussing potential issues that may arise going dimension up.


%For disk-like surfaces perhaps the most classical method to compute maps of this kind is the so called Tutte embedding~\cite{tutte1963draw}, which was proved back in 1963, and allows to compute $f_M : A \leftrightarrow B$ via barycentric mapping. This method is still used as basic ingredient to bootstrap robust methods for low distortion locally injective maps, which aim to minimize complex non linear energies and need a provably valid initial solution to start navigating  the feasible space towards a local minimum~\cite{rabinovich2017scalable}. 

%Sadly, it was shown multiple times via counter examples that the barycentric mapping does not extend to 3d~\cite{chilakamarri1995three,de2003tutte}. As of the time of writing, the problem of initializing a valid (i.e. locally injective) simplicial map between two topologial spaces of dimension $d \geq 3$ is still open. This problem has been widely investigated over the years, but the definition of a provably correct algorithm is still elusive, and even the most recent methods fail to provide guarantees of success~\cite{du2020lifting}.


%Despite this may seem just a tiny modification of our initial problem, this novel view allows to access a set of mature and well established tools that have never be used to attack the parameterization problem....



==> Earcut Mapping - A Mesh Generation Perspective on Robust Parameterizations/02_related.tex <==
\section{Background}
\label{sec:related}

In this section we discuss methods for robust surface mappings that are closest to us, also motivating why they cannot be extended to volumes.

The Tutte embedding~\cite{tutte1963draw} was introduced in 1963 in the context of graph drawing, and was popularized in the graphics community by Floater in 1997, showing that any convex combination of neighbor vertices can be used to define the map~\cite{floater1997parametrization}. Ever since, a plethora of different methods have been proposed in the field, extending the original idea to topological tori and disk-like meshes with multiple boundaries~\cite{gortler2006discrete}, as well as porting it to other spaces, such as Euclidean~\cite{aigerman2015orbifold}, hyperbolic~\cite{aigerman2016hyperbolic} and spherical~\cite{aigerman2017spherical} orbifolds. Despite numerous attempts, it was shown multiple times that the barycentric mapping does not extend to 3d. This is shown with a concise counter example in Figure~\ref{fig:tutte3dfail}; other failure cases are reported in~\cite{chilakamarri1995three,de2003tutte}. It is thought that under some restricting assumptions a 3d extension could still be possible~\cite{chilakamarri1995three}, but we are not aware of any success in this regard.

\begin{figure}
	\centering
	\includegraphics[width=.9\columnwidth]{img/tutte3dfail}
	\caption{Splitting a tetrahedron into four sub tets, and then splitting any of the so generated interior faces yields a simplicial complex with four boundary vertices (black) and two inner vertices (white). Fixing the boundary and solving for the Tutte's barycentric mapping~\cite{tutte1963draw} produces a mesh where edge $v_4v_5$ (in red) is collapsed, thus breaking the map.}
	\label{fig:tutte3dfail}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=.9\columnwidth]{img/collapse_fail}	
	\caption{Attempting to collapse the internal edges of a simple tetrahedralized sphere (left) along a random sequence always yields an incollapsible mesh where each edge violates the link condition~\cite{dey1998topology} (right). Applying barycentric subdivision allows to collapse new edges, but after each subdivision step the size of the incollapsible mesh we obtained was higher than the one at the iteration before.}
	\label{fig:incollapsiblesphere}
\end{figure}

The Tutte embedding offers theoretical guarantees but -- if pushed to the extreme -- concrete implementations may fail to produce a valid mapping because of the limited precision of floating point systems. Shen and colleagues propose an alternative method, called Progressive Embeddings~\cite{shen2019progressive}, which offers similar theoretical guarantees, but is less sensitive to floating point implementations. The algorithm is inspired by the progressive meshes concept~\cite{hoppe1996progressive}, and is based on the ability to deconstruct the topology of a triangle mesh by an ordered sequence of edge collapses, reconstructing the same mesh in another embedding with a sequence of vertex splits in the opposite order. Also this approach does not extend to 3d, the reason being twofold: (i) simplicial complexes in dimensions $d\geq 3$ may not be fully collapsible with a sequence of edge collapses, and even deciding whether a tetrahedral mesh is collapsible is NP Complete~\cite{tancer2016recognition,malgouyres2008determining,attali2014recognizing}. Theory says that after a finite set of barycentric subdivisions any simplicial complex becomes collapsible~\cite{adiprasito2019barycentric}, but still one should navigate the exponential space of all possible collapsing sequences to find a valid solution. Attempting to deconstruct a tetmesh along a heuristically computed collapsing sequence does not seem a good strategy either~\cite{lofano2019worst}. We personally tried many combinations of subdivisions and collapses, but always got stuck at some incollapsible configuration even on simple meshes (Figure~\ref{fig:incollapsiblesphere}); (ii) one may try to transform the input mesh into a mesh with different connectivity and known collapsing sequence via flip operators, but again this does not work because the graph of all possible triangulations of a given point set is connected for $d=2$~\cite{lawson1972transforming,osherovich2008all}, but there exist counter examples for the 3d case that show that it is disconnected for tetrahedralizations~\cite{dougherty2004unflippable}.
%for $d=3,4$ we do not know, while for $d\geq 5$ we know it is disconnected\cite[Chapter~7.3]{de2010structures}; 
All in all, these issues basically kill any hope that similar ideas could be extended to tetrahedral meshes in a robust yet computationally feasible manner. 

\begin{figure*}[h]
	\centering	
	\includegraphics[width=\linewidth]{img/pipeline}
	\caption{Our pipeline starts with two simple planar polygons (left). We the initialize two fronts (boundaries of the red shaded areas), which we progressively tessellate by adding triangles centered at front vertices that form valid ears (white circles) in both domains. Upon convergence, we obtain two meshes with same connectivity and different embedding (right).}
	\label{fig:example}
\end{figure*}

A variety of methods offer the ability to perform a cross parameterization between two surface meshes of same topology. They employ composition of maps to intermediate domains such as coarse base complexes~\cite{kraevoy2004cross,schreiner2004inter} or some polygonal schema~\cite{weber2014locally,Liv20,yang2020error}. These methods internally employ standard techniques (e.g. Tutte, or some derivation of it) to generate the underlying maps, therefore could potentially benefit from our contribution, and are orthogonal to it. 

Volume methods 
%For the volumes, many methods 
formulate the mapping as an optimization problem. As for the 2d case, topology is fixed in input, and differences arise in the energies and numerical schemes used. We count mainly two family of approaches: (i) methods that input an invalid map and project it into the feasible space by fixing inverted elements~\cite{aigerman2013injective,kovalsky2014controlling,su2019practical,du2020lifting}; (ii) methods that input a valid solution and iteratively reduce geometric distortion minimizing barrier energies that grow to infinity if an element becomes nearly degenerate or flips its orientation~\cite{rabinovich2017scalable}. The former do not provide any guarantee, and may fail to even enter the feasible space. The latter guarantee the generation of a valid map if correctly initialized. In 2d the initialization step can be computed with~\cite{tutte1963draw,shen2019progressive}. We are not aware of any 3d method that can provably generate a valid initial solution. 
%Robustly initializing a volumetric map is the ultimate goal and main motivation for the mesh generation approach proposed in this paper.

A simplified version of the volume mapping problem was proposed in~\cite{campen2016bijective}. This method is based on foliations, and allows to map a genus zero simplicial mesh to a cube or a sphere. Users can select the type of foliation (e.g. radial for the mapping to a sphere) but cannot prescribe point to point correspondences for surface vertices. Moreover, generating a valid piece-wise linear map requires to perform aggressive mesh refinement, greatly increasing output mesh size even for simple objects.

%These methods typically input an invalid map possibly containing degenerate or inverted elements, and cure it by relocating its vertices following the driving energy~\cite{}. Note that the optimization spaces in which they operate is highly non convex, and all these methods employ space convexification and sophisticated numerical schemes but cannot guarantee the generation of a valid map. A few months ago a novel method in this family was published~\cite{du2020lifting}, which seems very robust and for which a practical failure case has not be found yet. Still, theoretical guarantees can only be provided if the solution found by the optimizer is the global minimum of a complex functional, which cannot be computedcan be provided. The recent trend of flip preventing energies counts several methods that, if correctly inizialized with a valid solution, can greatly reduce geometric distortion without ever exiting the feasible space. These methods would greatly benefit from a mapping algorithm that provably provides a valid initial solution. To date, no method can provide it.


==> Earcut Mapping - A Mesh Generation Perspective on Robust Parameterizations/03_method.tex <==
\section{The Earcut Mapping Algorithm}
\label{sec:method}

In this section we introduce our novel surface mapping algorithm. We input two boundary representations of the domains $A$ and $B$ we want to connect in the form of two closed chains of vertices.
%, and output a bijective function $f : A \leftrightarrow B$. 
Domain $A$ is a simply connected planar region, possibly containing concavities. Domain $B$ must be strictly convex.
% Both domains are represented by two closed chains of vertices having the same number of elements, and not to contain any vanishing edge. 
If both chains do not contain vanishing edges there exists a one to one map $f_\partial : \partial A \leftrightarrow \partial B$. We extend such map from the boundary to the interior, providing in output a piece-wise linear function $f_M : M_A \leftrightarrow M_B$ in the form of two triangle meshes $M_A,M_B$ with same connectivity.% the  which can be navigated as described in Section~\ref{sec:intro}.

%Similarly to classical advancing front methods~\cite{lohner1996extensions,marcum1995unstructured}, our algorithm starts with a boundary mesh enclosing an empty domain, and genera

%As briefly stated in the introduction, 
Our key ingredient is a reformulation of the mapping problem in terms of mesh generation. We take inspiration from advancing front meshing algorithms such as~\cite{lohner1996extensions,marcum1995unstructured}, which start from a boundary (or initial front) describing an empty region to be meshed, and obtain the output mesh by progressively attaching new elements to such front, until it completely vanishes. Our key observation is that if we consider as initial fronts two regions we want to connect, and we define a sequence of advancing moves that are compatible with both fronts, we will obtain the same meshing for the two domains, hence a mapping between them. Compared to classical approaches, our special setting imposes three important differences:
\begin{itemize}
\item[1)] we work simultaneously in two domains, therefore advancing moves must be valid in both fronts, and must be applied following the same order;
\item[2)] at any time during execution, there must be a one to one correspondence between fronts in both domains, which must therefore be homotopic and contain the same number of vertices and edges;
\item[3)] assuming the absence of degenerate or flipped elements, \emph{any} meshing is ok, regardless of the quality of its elements. This differentiates from classical mesh generation algorithms, which largely concern about per element quality
\end{itemize}

The first condition ensures that all mesh elements we introduce have their own linear map connecting their two copies in both domains. The second condition ensures that the algorithm does not get stuck by creating topological mismatches in the fronts, which would prevent the completion of a valid global map. 
%Note that these are major constraints, and deeply impact the ability of known meshing algorithms to converge. They must be carefully taken into consideration when designing any new advancing front mapping algorithm. 
The third condition is just optional, but certainly applies to our case: we are only interested in initializing a valid map, without caring about geometric distortion. Methods that wish to generate a low distortion map may also leverage techniques for high quality advancing front mesh generation, but this is outside of the scope of this paper.

The algorithm works as follows: we initialize two fronts $F_A,F_B$ with the two input chains of vertices $A,B$. Since each domain is a simply connected polygon, we can use trivial earcut~\cite{eberly2008triangulation} to advance the front. Specifically, we detect convex front vertices in $F_A$ (i.e. vertices having inner angle lower than $\pi$), and check whether the triangle they form with their left and right neighbors contains any other vertex of $F_A$. If this is not the case, it means that the triangle is a valid ear, which can be \emph{cut} (i.e. removed) from the front, yielding a simpler polygon with one vertex less. Whenever a valid ear is found, the corresponding vertex is removed from both $F_A$ and $F_B$.
%. Specifically, we use trivial earcut~\cite{eberly2008triangulation}: we iteratively look for a valid ear in $F_A$, and generate a triangle centered at it both in $M_A$ and $M_B$. Each time a new ear is closed, the corresponding vertex is removed from $F_A,F_B$. 
Note that by our initial assumption $F_B$ is convex, hence any of its vertices forms a valid ear. Moreover, any ear cut from it will preserve its convexity, because removing a point from a convex polygon yields a simpler convex polygon. This greatly simplifies the meshing process, because it allows us to produce two meshes simultaneously by caring on the validity of each move only in one of the fronts ($F_A$). The iterative process continues as long as the size of the fronts is greater than 3. Once $\vert F_A \vert = \vert F_B \vert = 3$, we can complete the meshing by adding a triangle lid that vanishes both fronts. An algorithmic description of the method is given in Algorithm~\ref{alg}. Figure~\ref{fig:example} shows all the iterations for a simple example. 
%Figure~\ref{fig:teaser} shows a more complex mapping between a thickened space filling curve and a circle. 

\textbf{Convergence.} Decisions on which ear should be cut are always taken w.r.t. a single front ($F_A$). The problem is therefore equivalent to triangulating domain $A$, and convergence is guaranteed by the fact that any simple polygon has at least two valid ears~\cite{meisters1975polygons}, which is also the theoretical foundation for the earcut algorithm we employed. 
%Since everything is based on the triangulation of a simple polygon, the ear test is performed only in $F_A$, the process is guaranteed to converge. This is ensured by the famous theorem that states that any polygon 

\textbf{Complexity.} The complexity of the algorithm fully depends on the triangulation method of choice. For simplicity and ease of reproduction we opted for earcut. %implementation present in Cinolib~\cite{cinolib}. 
Despite optimal for a certain family of shapes~\cite{livesu2020deterministic}, the asymptotic complexity of this method for general simple polygons is
%of earcut for general polygons 
%Recent studies have shown that this algorithm is optimal (i.e. deterministic linear) on a restricted class of inputs, though on general simple polygons it has
 %$\mathcal{O}(n^3)$ if naively implemented, and can at most achieve 
 $\mathcal{O}(n^2)$~\cite{elgindy1993slicing,eberly2008triangulation}. Note that the mapping paradigm we propose is not strictly linked to earcut, which could be virtually substituted with any other triangulation algorithm, obtaining a different asymptotic complexity.
% which is well known for being not particularly efficient in the general case, 
%that earcut has only quadratic complexity, and may become optimal only when used on a narrower classes of simple polygons. For the sake of efficiency, any other triangulation method could be used instead, with no changes in the logic of the algorithm. 

%\textbf{Robustness.} The whole method is based around well established algorithms, and is guaranteed to converge to a valid solution for any input that fulfills our input requirements. Since any planar polygon can be triangulated without additional points, our mapping does not necessitate to add vertices in the meshes along the way. This makes the whole procedure extremely robust also from an implementative point of view, because no approximations introduced by the floating point system are possible. Besides the input point coordinates -- which are exact by definition -- the only computations involving floating points regard the diagonal test to detect valid ears in $F_A$. To this end, exact point in triangle tests based on robust geometric predicates~\cite{shewchuk1997adaptive} have been available in the meshing community since decades. All in all, this makes our algorithm robust without compromises, both theoretically and in practice.

\begin{algorithm}[t]
	\textbf{Input:} two closed lists of vertices $V_A, V_B$, such that both chains form simple polygons, $V_B$ is convex, and $\vert V_A \vert = \vert V_B \vert$.\\
ng a bijection $f_M : M_A \leftrightarrow M_B$\\
	%\giammi{il nome dell'algoritmo era addSegment, ma poi veniva chiamata la funzione addEdge. Ho uniformato tutto con addSegment}
	\hrulefill \\
	\SetAlgoLined
	\vspace{0.1em}
	$M_A = (V_A, \emptyset)$\;
	$M_B = (V_B, \emptyset)$\;
	initialize front $F_A$ with $V_A$\;
	initialize front $F_B$ with $V_B$\;
	\While{$\vert F_A \vert > 3$ }
	{
		find an index $i$ such that triangle $v_{i-1}, v_i, v_{i+1}$ is a valid ear in $F_A$\;
		insert triangle centered at $i$ in both $M_A$ and $M_B$\;
		$F_A = F_A \setminus i$\;
		$F_B = F_B \setminus i$\;
	}
	fill the triangular hole in $M_A$ with verts in $F_A$\;
	fill the triangular hole in $M_B$ with verts in $F_B$\;
	\textbf{return $M_A, M_B$}\;
	\caption{}
	\label{alg}
\end{algorithm}


\section{Extension to weakly visible polygons}
\label{sec:extension}
The algorithm presented in Section~\ref{sec:method} can only be used if one of the two domains is strictly convex. Mappings to non strictly convex polygons (e.g. a square) are not supported because if a triangle maps to three co-linear points it becomes degenerate. Similarly, concave polygons are not supported because they would require to validate each ear in both domains, possibly leading to deadlock configurations (Figure~\ref{fig:deadlock2d}).
%Mappings to non strictly convex domains are widely used by applications (e.g. for texture mapping and normal mapping) therefore 
In this section we discuss an extension of the mapping algorithm that permits mappings to any polygon that is weakly visible from an inner strictly convex domain~\cite{avis1981optimal,valentine1953minimal}. 
%This is a much bigger class of shapes, which fully contains convex polygons (both strict and non strict), star-shaped polygons, and even a portion of concave polygons that are non star shaped (Figure~\ref{}).
%to process a wider set of polygons. The method is quite general, and could potentially be applied 
%In this section we discuss a simple pre-processing routine that internally uses the same earcut approach, but extends it 

\begin{figure}
	\centering
	\includegraphics[width=.9\columnwidth]{img/fail2d}
	\caption{Failure case for Algorithm~\ref{alg}: the two polygons cannot be mapped to one another because convex vertices in the left star correspond to concave vertices in the right one, and vice versa. A mapping between the two stars is still possible if additional points are permitted, e.g. with the offsetting technique described in Section~\ref{sec:extension}.}
	\label{fig:deadlock2d}
\end{figure}

The basic idea is to split the mapping process in two parts. We first create an offsetting of the two domains, generating two sub polygons that live inside the input ones. One offset is generated with a topological approach, and can produce simple polygons of any shape. The other offset is computed with a geometric approach, and is guaranteed to produce a strictly convex polygon. Then, the mapping between offset polygons is generated with Algorithm~\ref{alg}, whereas the space in between offsets and the outer polygons is triangulated separately. In the remainder of this section we detail all the technical aspects of this modified pipeline.


%In particular, one polygon is offsetted using a topological method which can produce 
%offset the polygon inwards, generating an inner closed chain of vertices that has forms a strictly convex polygon. Doing so, the portion of the polygon contained inside the offset can be triangulated as described in the previous section, whereas the portion of the polygon in between the outer perimeter and the inner offset can be triangulated as detailed below.

\begin{figure*}
	\centering
	\includegraphics[width=\linewidth]{img/offsetting}
	\caption{Pipeline for our robust topological offsetting: (a) input polygon; (b) a triangulation of it; (c) splitting edges to ensure that each vertex has at least one incident edge not on the boundary; (d) adding offset points by splitting inner edges incident to each input vertex; (e) connecting the new vertices to form the inner chain; (f) completing the triangulation by adding quad diagonals. Exploiting the underlying mesh we can guarantee that the resulting offset does not self intersect, and that all formed triangles have consistent orientation.}
	\label{fig:offsetting}
\end{figure*}

\begin{figure*}
	\centering
	\includegraphics[width=\linewidth]{img/offset_mapping}
	\caption{Mapping the offsetted polygon shown in Figure~\ref{fig:offsetting} to a square: (a) we initialize a circle inside the square; (b) each outer point is mapped to the circle through the line connecting it with the circle center; (c) outer points that had multiple inner points introduce new samples in the circle, thus preserving strict convexity; (d) inner points are connected to form the offset polygon; (e) the space in between outer and inner polygons is triangulated.}
	\label{fig:offset_mapping}
\end{figure*}


\textbf{Topological offsetting.} Given a simple polygon $P$ with $n>3$ vertices, the topological offsetting produces a simple polygon $P'$ with $m \geq n$ vertices that is strictly contained in it. The offsetting procedure is depicted in Figure~\ref{fig:offsetting}: we firstly triangulate $P$, and then refine the so generated mesh in order to make sure that for each point $p \in P$ there is at least one incident edge that is not on the boundary. Since any simple polygon contains at least two valid ears~\cite{meisters1975polygons}, there will be at least two vertices with only two incident edges that require mesh refinement. Specifically, it can be proved that $\vert P' \vert \geq \vert P \vert +2$ for any polygon with five or more vertices. For each boundary vertex $p \in P$ we introduce as many offset points as the number of incident inner edges. We eventually connect these points in a closed loop, generating the wanted offset polygon $P'$. Working on an underlying triangulation gives great robustness to this method, which provides three important guarantees: (i) offset points are always positioned strictly inside the input polygon, because they sample inner edges in the triangulation; (ii) the offset polygon is topologically simple and forms a closed chain of vertices. Consistent vertex ordering is guaranteed by the underlying mesh topology; (iii) the offset polygon does not self intersect, because its sides can all be formed by splitting edges in the underlying triangulation.

\textbf{Geometric Offsetting.} The goal of this step is to reproduce the polygon obtained with topological offsetting in the second domain, ensuring that the result is a strictly convex polygon. 
%In this way, Algorithm~\ref{alg} can be applied to map the interior of the two offsets, whereas the triangulation of the space in between the input and offset polygons will be created as described thereafter. 
The geometric offsetting algorithm inputs a polygon $P$ and a disk $D \subset P$ with radius $r$ and center $c$. We assume that any corner of $P$ sees a portion of $D$, including its center. In other words, $D$ is \emph{weakly visible} from $P$~\cite{avis1981optimal,valentine1953minimal}. Note that weak visibility is a less restricting assumption than star shapedeness, hence $D$ must no be strictly contained in the kernel of $P$, although our geometric construction requires that at least its center $c$ does.
%In principle there's no need for $D$ to be a circle, any convex polygon would suffice, but to keep the interface of the software simple in our implementation we input a disk in the form of parameters $c,r$. 
The first step of the algorithm is to map each corner of $P$ onto $D$, computing the intersection between $D$ itself and the line connecting the corner with center $c$. These points already define a convex offset polygon with size $\vert P \vert$. However, topological offsetting generates polygons with bigger size, %(Figure~\ref{fig:offsetting}),
%associates more than one offset point to some of the vertices of $P$ , 
therefore we need to sample disk $D$ at some extra point to ensure that both offsets have the same number of vertices and same ordering. Let $p_i,p_{i+1} \in P$ be two adjacent points in the outer polygon, and $p_i',p_{i+1}' \in D$ the two offset points associated to them. We assign to point $p_i$ the circular arc delimited by $p_i',p_{i+1}'$, and use it to sample additional offset points that may be needed to match the topological offset obtained in the other domain. Additional points are generated so as to uniformly sample the first half of the arc. We leave the second half of the arc empty in order to avoid flips in the triangulation (Figure~\ref{fig:offset_half_angle}). Once all necessary points have been added, the geometric offset will contain the wanted number of vertices and be strictly convex, because all its points have been sampled on the input disk $D$.



\begin{figure}
	\centering
	\includegraphics[width=.9\linewidth]{img/offset_half_angle}
	\caption{Inserting additional vertices in the inner circle interpolating the angle between adjacent points may produce fold overs if the whole angle extent is used (left). Considering only half of the available angle allows to easily and robustly insert all the necessary points (right).}
	\label{fig:offset_half_angle}
\end{figure}

\textbf{Triangulation.} We compute a compatible triangulation of the space in between the outer polygon and its inner offset as follows.
%To complete the mapping, a compatible triangulation need be generated. Denoting with $A,B$ the two input polygons and with $A',B'$ their topological and geometric offsets, respectively, the interior of the offset polygons and the spaces $A \setminus A'$ and $B \setminus B'$ are triangulated separately. For the former, we exploit the fact that $A'$ is a general simple polygon and $B'$ is strictly convex, and we produce a compatible triangulation using the earcut mapping algorithm presented in the previous section. For the rest of the domain, we produce triangles as follows. 
Let us focus on polygon $A$ and its offset $A'$; the same triangulation scheme applies to $B,B'$ as well. Let $p_i \in A$ a vertex in the outer polygon, and $p'_{i,1},\dots,p'_{i,n} \in A'$ the offset points that are associated to it. We first generate $n-1$ triangles connecting adjacent offset vertices with $p_i$, forming triangles $p_i,p'_{i,j},p'_{i,j+1}$ for any $j = 1,\dots,n-1$. Then, we triangulate the remaining quads formed by vertices $p_i,p_{i+1},p'_{i,n},p'_{i+1,1}$ by tracing the diagonals $p_{i+1},p'_{i,n}$. The result of this triangulation can bee seen at the rightmost column of Figures~\ref{fig:offsetting} and~\ref{fig:offset_mapping}. We eventually complete the map by exploiting the fact that offset $B'$ is a strictly convex polygon, hence we run Algorithm~\ref{alg} using offsets $A'$ and $B'$ as input. 
% Merging these triangles with the compatible triangulation of $A',B'$ completes the meshing and thus the map.


==> Earcut Mapping - A Mesh Generation Perspective on Robust Parameterizations/04_results.tex <==
\begin{figure}
\centering
\includegraphics[width=.9\columnwidth]{img/space_filling/space_filling}
\caption{Mapping of a space filling curve to a circular (top), squared (middle) and star-shaped (bottom) domain. Triangles are colored from white to red according to the logarithm of their $\ell_2$ stretch~\cite{sander2001texture}.}
\label{fig:space_filling}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=.19\columnwidth]{img/dataset/beetle}
	\includegraphics[width=.19\columnwidth]{img/dataset/butterfly}
	\includegraphics[width=.19\columnwidth]{img/dataset/camel}
	\includegraphics[width=.19\columnwidth]{img/dataset/tree}
	\includegraphics[width=.19\columnwidth]{img/dataset/elephant}\\
	\includegraphics[width=.19\columnwidth]{img/dataset/stag}
	\includegraphics[width=.19\columnwidth]{img/dataset/splat}
	\includegraphics[width=.19\columnwidth]{img/dataset/spring}
	\includegraphics[width=.19\columnwidth]{img/dataset/crown}
	\includegraphics[width=.19\columnwidth]{img/dataset/lizzard}
	\caption{A sampling of the 2K shapes used in our experiments. For each model we produced three mappings: to a circle, a square and a star.}
	\label{fig:dataset}
\end{figure}


\section{Validation}
We implemented the earcut mapping and the offset algorithms in C++, and publicly released them as a module of CinoLib~\cite{cinolib}. We tested our algorithms on a MacBook Pro with an i5 2.9GHz processor and 16GB of RAM. For our tests, we collected a large dataset of shapes which comprises 1039 contours from the 2D shape structure dataset~\cite{carlier20162d}, and 1000 splat-like random polygons procedurally generated using Blender~\cite{blender} (Figure~\ref{fig:dataset}). For each shape in our benchmark we produced three alternative mappings: to a circle, a square, and a star-shaped domain (Figure~\ref{fig:space_filling}). Overall, we counted 2039 different shapes, and 6117 mappings. In all cases, our algorithms produced a valid (i.e. bijective) map, which we verified using exact orientation predicates~\cite{shewchuk1997adaptive}. Maps to circles involve only the earcut mapping Algorithm~\ref{alg}, and took 0.4 seconds overall. Maps to squares and stars also require topological and geometric offsetting, and took 3.77 and 3.68 seconds, respectively.

These experiments were particularly useful to give us insight on the  practical robustness of a floating point implementation. We soon observed that if the triangulation used to guide the topological offsetting contained elongated -- nearly degenerate -- triangles, then issues related with numerical precision could occasionally introduce flipped elements (Figure~\ref{fig:earcut}). This happened on approximately 100 mappings out of 6117.
%the topological offsetting described in Section~\ref{sec:extension} suffered from issues related with numerical precision when the triangulation used to guide the offsetting contained elongated quasi degenerate triangles. In the first implementation we were using standard earcut, which processes ears in the order they are found and may indeed introduce badly shaped triangles . With this code, around 100 mappings out of 6135 contained inverted elements.
From a mesh generation perspective this is not surprising at all: the most critical step in any mesh generation pipeline consists in placing additional points in the domain, because their coordinates must \emph{snap} to numbers that are representable in the floating point system, possibly introducing roundoff  errors. %Since our mapping procedure is based on mesh generation, it also suffers from the same weaknesses. 
We resolved this issue using a modified version of earcut that prioritizes its ears according to their inner angle, thus producing better triangulations and ultimately permitting us to successfully process all the models in our dataset. We can conclude that with this tiny modification the algorithm is robust both in theory and in practice, without necessitating the additional overhead of exact point coordinates kernels~\cite{CLSA20}.

%practical robustness of our algorithm. As it is well known in mesh generation literature, the most complex ingredient in a meshing pipeline is the handling of additional points, whose coordinates must be rounded in order to be representable in the machines' floating point system. To this end, we observed that 
%Despite formally correct, this extensive validation campaign gave us the possibility to address the practical robustness our algorithms. In particular, mappings to squares and stars, where the offsetting procedure is used, revealed that the topological offsetting may suffer from roundoff errors if the guiding triangulation of the domain contains almost degenerate elements. In our tests, using standard earcut




\begin{figure}
\centering
\includegraphics[width=\columnwidth]{img/earcut/earcut}
\caption{Top: topological offsetting is sensitive to extremely low quality guiding meshes, because offset points sample the edges of nearly degenerate triangles, possibly introducing degenerate or flipped elements due to numerical roundoff errors. Bottom: using a higher quality triangulation makes the algorithm numerically stable. In practice, we substituted classical earcut, which processes ears in the order they are found (top), with a prioritized earcut, which orders ears according to their angle (bottom).}
\label{fig:earcut}
\end{figure}

\section{Extension to Volumes}
\label{sec:3dmaps}
Besides its practical utility for 2D mappings, a major source of interest for this research deals with a volumetric extension of the algorithms proposed in Sections~\ref{sec:method} and~\ref{sec:extension}, in some way. In this section we analyze the major differences and challenges that we foresee.
%speculate about two possible future directions, namely: a tentative extension of the earcut method to volumes, and the possibility to extend the mapping method to pairs of non convex domains, both in 2d and 3d.

%To this end, we observe that there are mainly two challenges to overcome, namely the fact that earcut does directly apply to volumes, and the necessity of having additional Steiner points in the domain to even grant the existence of a tetrahedralization of a given triangle mesh enclosing a simple domain. In the following subsections we analyze both aspects.

\textbf{Convexity and Volumetric Earcut.}
In 2d the action of cutting an ear amounts to remove a convex vertex, substituting it with a straight segment that connects its two neighbors. Not only this operation is uniquely defined (there is one line passing through two given points), but it also decreases the inner angle of the neighbor vertices, preserving their convexity and, in turn, the convexity of the entire domain (if originally present). In 2d we deliberately exploit this property to restrict the quest for the next valid advancing move to one front only. For volumes, the situation is equivalent if and only if the convex vertex has valence 3. In such a case, cutting an ear amounts to delete the vertex, substituting it with a plane that interpolates its three neighbors, which is uniquely defined as well. This operation preserves the convexity of the domain, because dihedral angles can only decrease, and is the perfect dual of its 2d counterpart. Unfortunately, if the number of neighbors is higher than 3 (which is the most typical case for simplicial meshes) the operation of cutting an ear is not well defined, because the neighbor vertices may not be coplanar, and -- even if they were -- there would be multiple ways to triangulate them. One may still think to remove the vertex and triangulate the so generated pocket (some interesting ideas on how to tessellate these regions can be found in~\cite{chazelle1994bounds}), but if the neighbors are not coplanar some of the possible tessellations will not preserve convexity, which is a crucial property for the algorithm, and some other tessellations may not be applicable to the other domain, causing a deadlock. These observations suggest that domain convexity may be challenging to preserve throughout the mapping process, hence the ability to handle mappings to non convex domains must be devised. 


% Considering the non uniqueness of the volumetric earcut operator, the fact that some tessellations do not preserve convexity, and the fact that some other configurations may not be applicable in the starting (possibly non convex) domain, there may be configurations where the moves that are valid in one front are not valid for the other, causing a deadlock. This suggest two important aspects of a hypothetical 3d extension:
%\begin{itemize}
%\item the convexity of a domain may be hard (if not impossible) to preserve throughout the mapping process, hence the ability to handle two non convex domains must be devised;
%\item the insertion of additional points that allow to unlock possible deadlock configurations must be provided.
%\end{itemize}

% We believe that the basic idea could still be ported to volumes, but a well defined ear cutting strategy that must be devised, possibly involving the insertion of new points in the domain, which ensure both convexity and uniqueness. To this end, it becomes crucial to devise methods that provably require a finite number of additional points --  granting converge in a finite number of steps -- and are also numerically stable (e.g. when defining the coordinates of the newly generated points).

\textbf{Deadlocks and Steiner Points.}
%Another appealing extension of the mapping algorithm presented in Section~\ref{sec:method} regards the ability to generate maps between two non convex shapes, either planar or volumetric. Interestingly, both extensions raise the same crucial challenge, which is the necessity to insert additional (Steiner) points in the domains to complete the meshing.
Another important difference between 2D and 3D mesh generation is the ability to design a tessellation without inserting additional points in the domain. This is always possible in 2D~\cite{meisters1975polygons}, but not in 3D. For the volumetric case vertex insertion is a classical problem, and indecomposable polyhedra that cannot be tetrahedralized without Steiner points were already known almost one century ago~\cite{schonhardt1928zerlegung}. %Conversely, any planar domain can provably be triangulated without Steiner points~\cite{meisters1975polygons}, but in our specific setting it is easy to verify that even two copies of a simple polygon with different vertex rotations do not admit a compatible remeshing, which instead can be found by inserting additional points inside the domain (Figure~\ref{fig:deadlock2d}).

%Vertex insertion has been widely studied and -- from a theoretical standpoint  -- the topic is largely understood~\cite{goerigk2015indecomposable}. In practice, since computer programs often operate on numerical systems with finite precision, even the most advanced software available rely on heuristics for the computation of the coordinates of newly generated points, making this a critical step in any geometry processing pipeline~\cite{CLSA20}.


%In this section we speculate on a possible extension of the algorithm presented in Section~\ref{sec:method} to the third dimension. To this end, we observe that there is a big obstacle to overcome: in 2d the existence of a triangulation is guaranteed by a theorem that states that any simple polygon has at least two valid ears~\cite{meisters1975polygons}; in 3d the existence of such ears is not guaranteed, and there exist a variety indecomposable polyhedra that cannot be tetrahedralized as is, but necessitate additional special points in the domain~\cite{goerigk2015indecomposable}. 

%The necessity to add points in the domain to complete the mesh heavily affects our approach, which in Section~\ref{sec:method} assumed the convexity of one front across all iterations to greatly simplify the algorithm, permitting us to validate each move just in one of the two domains. 

%Advancing two fronts simultaneously in two non convex domains requires to always verify the validity of each move in both of them, with increased chances to get stuck in a deadlock configuration where no further move is possible. 
%Note that deadlock configurations may arise also in 2d, e.g. when both domains are non convex and the intersection of all valid moves is empty (Figure~\ref{fig:deadlock2d}). 
Indeed, Steiner points could be used to tetrahedralized indecomposable input domains, and also to unlock deadlock configurations when both domains are non convex. However, 
%These cases can be unlocked by inserting additional Steiner points (Figure~\ref{fig:deadlock2d}, bottom), but 
this re-opens a number of classical computational geometry questions that were answered for the meshing of a single domain and -- to the best of our knowledge -- have no answer for the special case of compatible meshing of two domains at once. Specifically:
%All these cases necessitate the insertion of additional Steiner points in both domains to permit to advance the front, raising a number of interesting computational geometry questions:

\begin{itemize}	
\item in case of a deadlock caused by two fronts that are indecomposable polyhedra, is it always possible to create a new move by adding one Steiner point in each domain? If not, what is the bound in the number of Steiner points that are necessary to grant the existence of a new valid move to advance both fronts simultaneously?\\

\item what if the deadlock is caused by the empty intersection between the valid moves in the two fronts, but considering each front alone a move exists? Is this case analogous to the point before?\\

\item what is the best positioning of a Steiner point in the context of simultaneous advancing front meshing? Can the coordinates of such point be expressed by rational numbers? This has huge practical importance, because it would guarantee that these points could be correctly positioned by a computer program (this is not the case for irrational numbers)\\

\item is there a bound on the global number of Steiner points necessary to simultaneously triangulate two polyhedra? For single volumes, we know from theory that this number is bounded by $\mathcal{O}(1)$ from below (see the Sch\"onhardt polyhedron~\cite{schonhardt1928zerlegung} and the subsequent generalization provided by Bagemihl~\cite{bagemihl1948indecomposable}), and by $\mathcal{O}(n^2)$ from above (by the Chazelle polyhedron~\cite{chazelle1984convex}). Should we expect similar bounds to exist also for pairs of shapes?\\
	
\item can we guarantee that compatible advancing front meshing always convergences?\\
\end{itemize}

Looking at previous literature for the meshing of a single domain we are tempted to be optimistic about the existence of reasonable (i.e. polynomial) bounds in the number of Steiner points, and the possibility to always unlock a deadlock configuration in $\mathcal{O}(1)$. Nevertheless, precise and theoretically sound answers to all these questions should be provided in order to grant robust tools for the generation of volumetric or non convex planar mappings.

%While these and many more questions have already been answered for single domains, the compatible remeshing of two domains at once proposes again the same questions in a multi object fashion. To the best of our knowledge, the topic has not been considered yet by researchers in computational geometry, and this will be our major focus for further works on the topic.

% theoretical issues:
% complexity: is there a bound on the maximum number of steiner points? how does it compare to the one mesh case?
% does the method converge?
% practical issues:
% when no move is possible on both domains, is it always possible to find one adding one steiner point?
%  where do I put new points? can coordinates be always represented as floats?


% also providing robust methods to devise their coordinates (possibly dealing with the limitations imposed by the floating point system). 

%The insertion of additional points is a major issue in volumetric mesh generation, and there exists a huge amount of literature on it. Nevertheless, solid mesh generation algorithm still struggle with Steiner points, and their insertion is still seen as a dark art by many~\cite{}.


==> Earcut Mapping - A Mesh Generation Perspective on Robust Parameterizations/05_conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}
We have proposed a novel algorithm to generate maps between simple polygons. At the core of this article is the proposal of a novel paradigm for the robust generation of simplicial maps, which is rooted in the principles of compatible mesh generation. We assume the input to be just a boundary representation of the domains to be connected, and we consider the mesh connectivity as an additional unknown. We then formulate the mapping as a mesh generation problem, where one wants to construct the same mesh in two different embeddings. This differentiates from classical approaches, which assume the topology of the mesh to be fixed, and solve the problem of positioning the interior vertices of a given mesh inside target domain. To grant maximal adoption we publicly released a reference implementation of our algorithms in Cinolib~\cite{cinolib}.

As witnessed by our results, the algorithms we propose are both theoretically sound and practically robust, and cover a wider range of mapping domains than prior methods, which are limited to convex~\cite{tutte1963draw,shen2019progressive}. On the other hand, our tools can only be used in a 2D-to-2D fashion, because a closed curve unambiguously identify a topological space only in 2d. Prior methods input a pre-existing surface mesh, which can be embedded in any higher dimensional space, hence~\cite{tutte1963draw,shen2019progressive} can also be used in a 3D-to-2D fashion.

%Our method is both theoretically sound and practically robust, but has little practical relevance because equally robust methods were already known for the 2d case 
We are mainly interested in this novel paradigm because it opens to a possible extension to volumetric meshes. This is a major difference w.r.t. prior art, because existing robust 2D approaches cannot extend to 3d (Section~\ref{sec:related}). To this end, in the final part of the paper we discussed potential issues that arise going one dimension up, and revived a number of classical computational geometry questions that are already answered for the meshing of a single domain, but have no answer for the novel case of compatible meshing. We believe that answering these questions will provide powerful tools to attack the volumetric mapping problem via mesh generation, and we will devote our future works to further develop this line of research. At the moment it is impossible to say whether a 3D extension would be computationally feasible, but the literature and wide availability of efficient tools for volume mesh generation leaves us reasonable hopes that in the near future a mapping method of this kind could be implemented.

%\cino{limitations: } Note that differently from Tutte and Progressive Embeddings, which are tailored for convex domains only, our method achieves comparable robustness on a wider class of 2D domains, allowing us to map complex shapes like a space filling curve to a star (Figure~\ref{fig:space_filling}). However, our method can only be used for planar mappings, because our input is a closed curve that must unambiguously enclose a polygon. Conversely, methods like Tutte and Progressive Embeddings input a mesh and a target (planar) domain, hence can be used to flatted a topological disk embedded in $\mathbb{R}^3$ onto the plane.


%were already answered for the meshi
% regarding the insertion of Steiner points in the domains. This is a classical computational geometry topic which has been widely studied in the past. To the best of our knowledge, there are no works that look at the problem from a compatible meshing point of view. It is therefore our intent to further study the topic, in the hope that this will pave the way for a new algorithmic approach to the volumetric mapping problem.

%considering two non convex domains (both in 2d and 3d) raises a number of additional challenges that depend from the necessity to insert Steiner points in the domains. This is a classical topic in computational geometry, but the simultaneous insertion of Steiner points in multiple domains have 
%
%in lifting this algorithm one dimension above, to produce volumetric maps between two tetrahedral meshes. Differently from prior planar methods such as Tutte~\cite{tutte1963draw} and Progressive Embeddings~\cite{shen2019progressive}, which suffer from major theoretical issues in 3d, our mesh generation approach seems to permit an extension to 3d. 



==> Earcut Mapping - A Mesh Generation Perspective on Robust Parameterizations/99_utilities.tex <==
%%%%%%%%%%%%
% USEFUL COMMANDS
%%%%%%%%%%%%

\newcommand{\cino} [1]{{\color{magenta}	Cino: #1}}
\newcommand{\com} [1]{{}} % comment stuff out....
\newcommand{\edit} [1]{{\color{black}			#1}} % mark edits in red (e.g. after a revision)

\newcommand{\M}{M} % manifold
\renewcommand{\l}{\ell} % loop
\renewcommand{\P}{P} % polygon
\newcommand{\Q}{Q} % queue
\newcommand{\genus}[1]{{ g( #1 ) }}% genus

